Adversarial Attacks on Variational Autoencoders

Adversarial attacks are malicious inputs that derail machine-learning models. We propose a scheme to attack autoencoders, as well as a quantitative evaluation framework that correlates well with the qualitative assessment of the attacks. We assess --- with statistically validated experiments --- the resistance to attacks of three variational autoencoders (simple, convolutional, and DRAW) in three datasets (MNIST, SVHN, CelebA), showing that both DRAW's recurrence and attention mechanism lead to better resistance. As autoencoders are proposed for compressing data --- a scenario in which their safety is paramount --- we expect more attention will be given to adversarial attacks on them.

==> extra-material.tex <==
The seminal article of Szegedy \emph{et al.} \cite{szegedy2013intriguing} introduced adversarial images, showing how to force a deep network to misclassify an image by applying nearly imperceptible distortions. Goodfellow \emph{et al.} \cite{goodfellow2014explaining} exploited the linear nature of deep convolutional networks to both attempt explaining how adversarial samples arise, and to propose a much faster technique to create them. Tabacof and Valle \cite{tabacof2015exploring} explored the geometry of adversarial regions, showing that they appear in relatively dense regions of the input space, and that shallow, simple classifiers tend to be more robust to them.

The existence of adversarial images lead to interesting questions on their significance, and even usefulness. Training models to resist adversarial attacks was advanced as a form of regularization~\cite{goodfellow2014explaining, miyato2015distributional}. Gu \emph{et al.} \cite{gu2014towards} used autoencoders to pre-process the input and try to reinforce the network against adversarial attacks, finding that although in some cases resistance improved, attacks with small distortions remained possible. A more recent trend is training adversarial \emph{models}, in which one attempts to generate “artificial” samples (from a generative model) and the other attempts to recognize those samples~\cite{goodfellow2014generative}. Makhzani \emph{et al.} \cite{makhzani2015adversarial} employ such scheme to train an autoencoder.

Here, we explore adversarial images for autoencoders — models optimized to reconstruct their inputs from compact internal representations. In an autoencoder, the attack targets not a single label, but a whole reconstruction. 


\begin{figure}[ht!]
      \centering
      \begin{subfigure}[b]{0.45\textwidth}
          \includegraphics[width=\textwidth]{graphs/mnist_exp_1.png}
          \label{fig:MNIST_VAE_Example_Dist}
      \end{subfigure}
      \begin{subfigure}[b]{0.45\textwidth}
          \includegraphics[width=\textwidth]{graphs/mnist_exp_1_imgs.png}
          \label{fig:MNIST_VAE_Example}
      \end{subfigure}
      \begin{subfigure}[b]{0.45\textwidth}
          \includegraphics[width=\textwidth]{graphs/svhn_exp_6.png}
          \label{fig:SVHN_VAE_Example_Dist}
      \end{subfigure}
      \begin{subfigure}[b]{0.45\textwidth}
          \includegraphics[width=\textwidth]{graphs/svhn_exp_6_imgs.png}
          \label{fig:SVHN_VAE_Example}
      \end{subfigure}
      \begin{subfigure}[b]{0.45\textwidth}
	          \includegraphics[width=\textwidth]{graphs/exp_0.png}
          \label{fig:CELEBA_VAE_Example_Dist}
      \end{subfigure}
      \begin{subfigure}[b]{0.45\textwidth}
          \includegraphics[width=\textwidth]{graphs/exp_0_imgs.png}
          \label{fig:CELEBA_VAE_Example}
      \end{subfigure}
      \caption{[TODO] Top row: MNIST. Bottom row: SVHN. The figures on the left show the trade-off between the quality of adversarial attack and the adversarial distortion magnitude, with changing regularization parameter (implicit in the graphs, chosen from a logarithmic scale). The figures on the right correspond to the points shown in red in the graphs, illustrating adversarial images and reconstructions using fully-connected, and convolutional variational autoencoders (for MNIST and SVHN, respectively).}
      \label{fig:attackExamples}
\end{figure}

\begin{comment}
\begin{figure}[ht!]
      \centering
          \includegraphics[width=0.7\textwidth]{auc_example.png}
      \caption{The proposed metric: Area Under the Distortion--Distortion Curve (AUDDC).}
      \label{fig:auc}
\end{figure}
\end{comment}


\begin{comment}
We can choose the attacker's regularization parameter $C$ in classification tasks by bisection as the smallest value which still misleads the model~\cite{tabacof2015exploring}. However, we cannot do same for autoencoders, since we don't have a binary criterion for success. Therefore, we are going to use the method Tabacof and Valle introduced in their previous work~\cite{tabacof2016advvae} where they forgo a determination of one single point and compute the whole Distortion--Distortion curve. For that

To create a baseline, we use a similar method to generate a range of adversarial images for the classification task on the MNIST and SVHN dataset (CelebA was not used because its images have multiples attributes to be identified and not general classes) with the intent to contrast the behavior of the adversarial attacks across the two task (classification and autoencoding). We pick pairs of original image / adversarial class (axis “experiment”), and varying $C$ (from $2^{-10}$ to $2^{20}$), we measure the distortion as above, and the probability (with  corresponding logit) attributed to the adversarial (blue  scatter) and to the original classes (green scatter). The axes here are no longer normalized, but we center at 0 in the ``distortion'' axis the transition point between attack failure and success --- the point where green and blue lines cross.

Important to note that  encoder's and decoder's parameters ($\phi$ and $\theta$) remain constant during the adversarial optimization. 

[TODO: find a place for those technicalities =>]  Another common constraint is making sure that the images stay within their valid space (i.e., no pixels “below black or above white”). In the cases where an optimization problem is created, it is common to use L-BFGS or Adam~\cite{kingma2014adam} to solve it~\cite{carlini2016towards}. However, other techniques can be used, for instance, the fast gradient sign~\cite{goodfellow2014explaining}.
\end{comment}

% with only one timestep without the attention mechanism; 4) DRAW with only one timestep with the attention mechanism; 5) DRAW with 16 timesteps without the attention mechanism; and 6) DRAW with 16 timesteps with the attention mechanism. We used models with 32 and 128 latent variables for MNIST and SVHN and 256 and 2048 latent variables for CelebA. Since DRAW has a unique latent space where each timestep has its own set of latent variables, we are considering that total number of latent variables in a DRAW model is product between the number of latent variables and the number of timesteps. For instance, a DRAW model with 128 latent variables and 16 timesteps is considered to have a total 2048 latent variables.



\begin{comment}
Consider a classifier $\bm{p} = f(\bm{x})$ that, for each input image $\bm{x}$, outputs a vector of probabilities where ${p}_{i}$  corresponds to the probability of the given image having a corresponding label $i$. $L$ and $U$ are the lower and upper bounds of the image pixel space. The idea is to add the smallest distortion $D$ to $X$, such that
the highest label probability given by $\argmax_i \bm{p} = {f(\bm{x}+\bm{d})}$ will no longer be assigned to $X$'s original class, thus causing $X$ to be misclassified, as shown in the optimization problem \cite{szegedy2013intriguing,tabacof2015exploring}:

\begin{equation}
\begin{aligned}
& \underset{\bm{d}}{\text{minimize}}
& & \| \bm{d} \| + C\cdot\xentropy(\bm{p}, \bm{p^A})\\
& \text{subject to}
& & L \leq \bm{x} + \bm{d} \leq U \\
& & & \bm{p} = f(\bm{x}+\bm{d}) \\
\end{aligned}
\label{eq:min}
\end{equation}

It is also possible to linearize the classifier around its operating point (i.e. the input image) and use an infinity-norm constraint in order to guarantee small pixel changes. This leads to fast gradient sign method \cite{goodfellow2014explaining}:

\begin{equation}
\begin{aligned}
& \bm{d} = \epsilon sign(\delta_{\bm{x}}J(\theta, \bm{x}, y))
\end{aligned}
\label{eq:fast}
\end{equation}
\end{comment}
\begin{comment}
\begin{figure}[h!]
      \centering
      \begin{subfigure}[b]{0.45\textwidth}
          \includegraphics[width=\textwidth]{MNIST_adv_vae_example_dist.png}
          \label{fig:MNIST_VAE_Example_Dist}
      \end{subfigure}
      \begin{subfigure}[b]{0.45\textwidth}
          \includegraphics[width=\textwidth]{MNIST_adv_vae_example.png}
          \label{fig:MNIST_VAE_Example}
      \end{subfigure}
      \begin{subfigure}[b]{0.45\textwidth}
          \includegraphics[width=\textwidth]{SVHN_adv_vae_example_dist.png}
          \label{fig:SVHN_VAE_Example_Dist}
      \end{subfigure}
      \begin{subfigure}[b]{0.45\textwidth}
          \includegraphics[width=\textwidth]{SVHN_adv_vae_example.png}
          \label{fig:SVHN_VAE_Example}
      \end{subfigure}
      \caption{Top row: MNIST. Bottom row: SVHN. The figures on the left show the trade-off between the quality of adversarial attack and the adversarial distortion magnitude, with changing regularization parameter (implicit in the graphs, chosen from a logarithmic scale). The figures on the right correspond to the points shown in red in the graphs, illustrating adversarial images and reconstructions using fully-connected, and convolutional variational autoencoders (for MNIST and SVHN, respectively).}
      \label{fig:AdvExamples}
\end{figure}

We found that generating adversarial images for autoencoders is a much harder task than for classifiers. If we apply little distortion (comparable to those used for misleading classifiers), the reconstructions stay essentially untouched. To get reconstructions very close to the target's, we have to apply heavy distortions to the input. However, by hand-tuning the regularization parameter, it is possible to find trade-offs where the reconstruction approaches the target's and the adversarial image will still resemble the input (two examples in Fig. \ref{fig:AdvExamples}).

%By varying the regularization parameter $C$, the generated adversarial image has more or less distortion. As $C$ increases, the adversarial image has less distortion and its distance to the original image tends to decrease while the distance of the adversarial image's reconstruction to the target image tends to increase.

The plots for the full set of 25 original/target image pairs appear in Fig.~\ref{fig:Adv_3D}. All series saturate when the latent representation of the adversarial image essentially equals the target's. That saturation appears well before the upper distortion limit of 1.0, and provides a measure of how resistant the model is to the attack: Variational Autoencoders appear slightly more resistant than Deterministic Autoencoders, and MNIST much more resistant than SVHN. The latter is not surprising, since large complex models seem, in general, more susceptible to adversarial attacks.  Before the “hinge” where the attack saturates, there is a quasi-linear trade-off between input distortion and output similarity to target, for all combinations of dataset and autoencoder choice. We were initially hoping for a more non-linear behavior, with a sudden drop at some point in the scale, but data suggests that there is a give-and-take for attacking autoencoders: each gain in the attack requires a \emph{proportional} increase in distortion. 

\begin{figure}[h]
      \centering
      \begin{subfigure}[b]{0.45\textwidth}
          \includegraphics[width=\textwidth]{MNIST_adv_vae_3D_mean.png}
          \label{fig:MNIST_VAE_3D}
      \end{subfigure}
      \begin{subfigure}[b]{0.45\textwidth}
          \includegraphics[width=\textwidth]{SVHN_adv_vae_3D_mean.png}
          \label{fig:SVHN_VAE_3D}
      \end{subfigure}
      \begin{subfigure}[b]{0.45\textwidth}
          \includegraphics[width=\textwidth]{MNIST_adv_ae_3D.png}
          \label{fig:MNIST_AE_3D}
      \end{subfigure}
      \begin{subfigure}[b]{0.45\textwidth}
          \includegraphics[width=\textwidth]{SVHN_adv_ae_3D.png}
          \label{fig:SVHN_AE_3D}
      \end{subfigure}
      \caption{Plots for the whole set of experiments in MNIST and SVHN. Top: variational autoencoders (VAE). Bottom: deterministic autoencoders (AE). Each line in a graph corresponds to one experiment with adversarial images from a single pair of original/target images, varying the regularization parameter $C$ (like shown in Fig.~\ref{fig:AdvExamples}). The “distortion” and “adversarial$-$target” axes show the trade-off between cost and success. The “hinge” where the lines saturate show the point where the reconstruction is essentially equal to the target's: the distortion at the hinge measures the resistance to the attack.
      %Each curve represents the $\ell_2$ distances between the adversarial image and the original, as well as the $\ell_2$ distances between the adversarial reconstruction image and the target. The x-axis of each individual curve was normalized in order to $x=1$ represent the $\ell_2$ distance between the original and target images. The z-axis was normalized in order to $z=0$ represent the $\ell_2$ distance between the target and its reconstruction, and $z=1$ represent the $\ell_2$ distance between the the reconstruction of the original image and the target. The horizontal and vertical bars in Fig. \ref{fig:AdvExamples} visually display the bounds that are used to normalize one experiment.      
      }
\label{fig:Adv_3D}
\end{figure}
 
The comparison with the (much better-studied) attacks for classifiers, showed, at the beginning, a much different behavior: when we contrasted the probability attributed to the adversarial class \emph{vs.} the distortion imposed on the input, we observed the non-linear, sudden change we were expecting~(left column of Fig.~\ref{fig:clf_3D}). The question remained, however whether such non-linearity was intrinsic, or whether it was due to the highly non-linear nature of the probability scale. The answer appears in the right column of Fig.~\ref{fig:clf_3D}, where, with a logit transformation of the probabilities, the linear behavior appears again. It seems that the attack on classifiers show, internally, the same linear give-and-take present in autoencoders, but that the normalization of the outputs of the last layer into valid probabilities aids the attack: changes in input lead to proportional changes in logit, but to much larger changes in probability. That makes feasible for the attack on classifiers to find much better sweet spots than the attack on autoencoders (Fig.~\ref{fig:Adv_clf}). Goodfellow et al.~\cite{goodfellow2014explaining} suggested that the linearity of deep models make them susceptible to adversarial attacks. Our results seems to reinforce that such linearity plays indeed a critical role, with “internal” success of the attack being proportional to the distortion on inputs. On classification networks, however, which are essentially piecewise linear until the last layer, the non-linearity of the latter seems to compound the problem.

%. In fig. \ref{fig:Adv_clf} we see two examples, one for MNIST and one for SVHN, where we also vary the regularization parameter $C$ on a logarithmic scale. We can see when the image actually becomes adversarial on the crossing point of the two curves. We can see that the attack on the logit scale is linear, similar to the attack on the autoencoders. However, the output of the classifier is the transformation of the logit into valid probabilities. This non-linearity makes the linear change of the logit into a nonlinear change. This shows why adversarial attacks are very successful in classifiers: Changes in input lead to proportional changes in the logit, which in turn quickly change value in the probability. Since the classifier is fooled in the probability space, it is possible to find a point where a small increase in adversarial distortion will be enough to make the output change sides.

\begin{figure}[h!]
     \centering
     \begin{subfigure}[b]{0.35\textwidth}
         \includegraphics[width=\textwidth]{MNIST_clf_prob.png}
         \label{fig:MNIST_clf_prob}
     \end{subfigure}
     \begin{subfigure}[b]{0.35\textwidth}
         \includegraphics[width=\textwidth]{MNIST_clf_logit.png}
         \label{fig:MNIST_clf_logit}
     \end{subfigure}
     \begin{subfigure}[b]{0.125\textwidth}
         \includegraphics[width=\textwidth]{MNIST_clf_ex.png}
         \label{fig:MNIST_clf_ex}
     \end{subfigure}
     \begin{subfigure}[b]{0.35\textwidth}
         \includegraphics[width=\textwidth]{SVHN_clf_prob.png}
         \label{fig:SVHN_clf_prob}
     \end{subfigure}
     \begin{subfigure}[b]{0.35\textwidth}
         \includegraphics[width=\textwidth]{SVHN_clf_logit.png}
         \label{fig:SVHN_clf_logit}
     \end{subfigure}
     \begin{subfigure}[b]{0.125\textwidth}
         \includegraphics[width=\textwidth]{SVHN_clf_ex.png}
         \label{fig:SVHN_clf_ex}
     \end{subfigure}
     \caption{Examples for the classification attacks. Top: MNIST. Bottom: SVHN. Left: probabilities. Middle: logit transform of probabilities. Right: images illustrating the intersection point of the curves. The adversarial class is ‘4’ for MNIST, and ‘0’ for SVHN. The red curve shows the probability/logit for the adversarial class, and the blue curve shows the same for the original class: the point where the curves cross is the transition point between failure and success of the attack.} 
     \label{fig:Adv_clf}
\end{figure}

\begin{figure}[h!]
	\centering
 	\begin{subfigure}[b]{0.45\textwidth}
 		\includegraphics[width=\textwidth]{MNIST_clf_prob_3D}
 		\label{fig:MNIST_clf_prob_3D} 
     \end{subfigure}
	\begin{subfigure}[b]{0.45\textwidth}
		\includegraphics[width=\textwidth]{MNIST_clf_logit_3D}
		\label{fig:MNIST_clf_logit_3D} 
    \end{subfigure}
 	\begin{subfigure}[b]{0.45\textwidth}
 		\includegraphics[width=\textwidth]{SVHN_clf_prob_3D}
 		\label{fig:SVHN_clf_prob_3D} 
     \end{subfigure}
	\begin{subfigure}[b]{0.45\textwidth}
		\includegraphics[width=\textwidth]{SVHN_clf_logit_3D}
		\label{fig:SVHN_clf_logit_3D} 
    \end{subfigure}
	\caption{Plot of whose set of experiments for classifiers. Top: MNIST. Bottom: SVHN. Left: probabilities. Right: logit transform of probabilities. Each experiment corresponds to one of the graphs shown in Fig.~\ref{fig:Adv_clf}, centered to make the crossing point between the red and blue lines stay at 0 in the “distortion” axis.}
	\label{fig:clf_3D}
\end{figure}

%When we repeat the experiment on 25 different adversarial images for classifiers we see that the pattern holds: Due to the non-linearity set by the softmax output layer, there is always a quick phase change. Note that the change to the input to the softmax (logit) is similar to the autoencoder case. This shows that adversarial attacks are effective in classifiers because of this nonlinear relation in the output and that the change before the output is linear. This is evidence in favor of Goodfellow's hypothesis that the adversarialness is present in deep neural networks because of its linearity \cite{goodfellow2014explaining}.
\end{comment}

%\FloatBarrier 
%%% Conclusion %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Terminology:
\begin{itemize}
\item Original image: Image without the adversarial distortion
\item Adversarial image: Image with the adversarial distortion
\item Adversarial distortion: Difference between original and adversarial image
\item Adversarial loss: Function that captures the adversarialness of the adversarial image
\item Adversarial regularization: Function that limits the adversarial distortion to be minimal
\item Original label (classifiers): Class of the original image
\item Adversarial label (classifiers): Adversarial attack label objective
\item Adversarial input (autoencoders): Same as adversarial image
\item Target image (autoencoders): Adversarial attack reconstruction objective
\item Adversarial reconstruction(autoencoders): Reconstruction of the adversarial input
\end{itemize}

We worked on the binarized MNIST~\cite{lecun1998mnist} and SVHN datasets \cite{netzer2011reading}. The former allows for very fast experiments and very controlled conditions; the latter, while still allowing to manage a large number of experiments, provides much more noise and variability. Following literature~\cite{kingma2013auto}, we modeled pixel likelihoods as independent Bernoullis (for binary images), or as independent normals (for RGB images). We used Parmesan and Lasagne \cite{lasagne} for the implementation\footnote{The code for the experiments can be found at \url{https://github.com/tabacof/adv_vae}}.

The loss function to train the variational autoencoder (equation~\ref{eq:vae}) is the expectation of the likelihood under the approximated posterior plus the KL divergence between the approximated posterior and the prior. We approximate the expectation of the likelihood with one sample of the posterior. We extract the gradients of the lower bound using automatic differentiation and maximize it using stochastic gradient ascent via the ADAM algorithm \cite{kingma2014adam}. We used 20 and 100 latent variables for MNIST and SVHN, respectively. %The prior of the latent variables are independent normals, with zero mean and unitary variance. The approximated posterior is parameterized as an independent multivariate normal distribution with means and variances determined by the encoder network (see equation~\ref{eq:vae}), so the KL divergence has an analytical form \cite{kingma2013auto}
We parameterized the encoder and decoder as fully-connected networks in the MNIST case, and as convolutional and deconvolutional \cite{zeiler2010deconvolutional} networks in the SVHN case. After the training is done, we can use the autoencoder to reconstruct some image samples through the latent variables, which are the learned representation of the images.  An example of a pair of input image/reconstructed output appears in Fig.~\ref{fig:autoencoderDiagram}.

%We generate adversarial images for autoencoders. That is, we add adversarial distortion to a particular image to make its reconstruction by the autoencoder seem like another image. The adversarial image is the original image plus the adversarial distortion. The target image is what we want the reconstruction to look like. Our first strategy was the minimization of the difference between the reconstruction and the target image, plus a regularization term (L2 norm of the distortion). This did not work as intended and the reconstruction simply became blurred. A second strategy that achieved better results was the minimization of the KL divergence of the latent variables of the target image and the adversarial image (see equation~\ref{eq:vae_adv}), as shown in figure \ref{fig:advAutoencoderDiagram}. This lead to better results, though not quite as impressive as the adversarial images for classification.



\begin{table}[h]
\begin{equation}
\label{eq:vae_adv}
\noindent
  \thinmuskip=\muexpr\thinmuskip*5/8\relax
  \medmuskip=\muexpr\medmuskip*5/8\relax
\begin{aligned}
& \underset{\bm{d}}{\text{min.}}
& & KL\infdiv{\bm{z}_{target}}{\bm{z}_{adversarial}} + C\| \bm{d} \| \\
& \text{s.t.}
& & L \leq \bm{x}_{original} + \bm{d} \leq U \\
& & & \bm{z}_{target} \sim \mathcal{N}(\bm{\mu}_{\phi}(\bm{x}_{target}), \exp(\bm{\sigma}_{\phi}^2(\bm{x}_{target}))) \\
& & & \bm{z}_{adv} \sim \mathcal{N}(\bm{\mu}_{\phi}(\bm{x}_{original}+\bm{d}), \exp(\bm{\sigma}_{\phi}^2(\bm{x}_{original}+\bm{d}))) \\
\end{aligned}
\end{equation} 
\end{table}

Where $\bm{d}$ is the adversarial distortion, $\bm{x}_{original}$ is the original image, $\bm{x}_{original}+\bm{d}$ is the adversarial image, $\bm{z}$ are the latent variables, $\phi$ are the encoder parameters (i.e. weights), $L$ and $U$ are the bounds on the input space, and $C$ is the regularizing constant the balances the adversarial loss and the adversarial regularization.

We also tested inverting the KL-divergence order and using the L2 distance between the latent variables parameters (i.e., mean and standard deviation), with worse results.
Our first strategy was the minimization of the difference between the reconstruction and the target image. This did not work as intended and the reconstruction simply became blurred. 

In the case of regular autoencoders, the difference is captured by the L2 distance of the bottleneck layer values:

\begin{table}[h]
\begin{equation}
\label{eq:ae_adv}
\noindent
  \thinmuskip=\muexpr\thinmuskip*5/8\relax
  \medmuskip=\muexpr\medmuskip*5/8\relax
\begin{aligned}
& \underset{\bm{d}}{\text{min.}}
& & \| \bm{z_{target}} - \bm{z_{reconstruction}} \| + C\| \bm{d} \| \\
& \text{s.t.}
& & L \leq \bm{x}_{original} + \bm{d} \leq U \\
& & &  \bm{z_{reconstruction}} = encoder(\bm{x}_{original} + \bm{d})
\end{aligned}
\end{equation} 
\end{table}



For classification tasks, the regularization term $C$ (Eq.~\ref{eq:ae_adv}) may be chosen by bisection as the smallest constant that still leads to success~\cite{tabacof2015exploring}. Autoencoders complicate such choice, for there is no longer a binary criterion for success. Goodfellow \emph{et al.} \cite{goodfellow2014explaining} and Sabour \emph{et al.}\cite{sabour2015adversarial} optimize differently, choosing for $\Delta$ an $\ell_\infty$-norm constrained to make the distortion imperceptible, while maximizing the misdirection. We found such solution too restrictive, leading to reconstructions visually too distinct from the target images. Our solution was instead to forgo a single choice for $C$, and analyze the behavior of the system throughout a series of values.

In our experiments, we pick at random 25 pairs of original/target images (axis “experiment” in  graphs). For each pair, we span 100 different values for the regularization constant $C$ in a logarithmic scale (from $2^{-20}$ to $2^{20}$), measuring the $\ell_2$-distance between the adversarial input and the original image (axis “distortion”), and the $\ell_2$-distance between the reconstructed output and the target image (axis “adversarial$-$target”). The “distortion” axis is normalized between 0.0 (no attack) and the $\ell_2$-distance between the original and target images in the pair (a large distortion that could reach the target directly). The “adversarial$-$target” is normalized between the $\ell_2$-distance of the reconstruction of the target and the target (the best expected attack) and the $\ell_2$-distance of the reconstruction of the original and the target (the worst expected attack). The geometry of such normalization is illustrated by the colored lines in the graphs of Fig.~\ref{fig:AdvExamples}. For variational autoencoders, the reconstruction is stochastic: therefore, each data point is sampled 100 times, and the average is reported.

For comparison purposes, we use the same protocol above to generate a range of adversarial images for the usual classification tasks on the same datasets. The aim is to contrast the behavior of adversarial attacks across the two tasks (autoencoding / classification). In those experiments we pick pairs of original image / adversarial class (axis “experiment”), and varying $C$ (from $2^{-10}$ to $2^{20}$), we measure the distortion as above, and the probability (with  corresponding logit) attributed to the adversarial (red lines) and to the original classes (blue lines). The axes here are no longer normalized, but we center at 0 in the “distortion” axis the transition point between attack failure and success --- the point where red and blue lines cross.

%Even though there are efficient ways to find $C$ in the case of adversarial images for classifiers, we also create adversarial images for classifiers with a varying $C$ using the same datasets (gray-scale MNIST and SVHN), using a two layered fully-connected network and a convolutional network, respectively. This can be used to compare the tasks of adversarial images for autoencoders and for classifiers. If the trade-off between adversarial distortion and adversarial loss is different, then we show that there are intrinsic differences between the tasks. Following Goodfellow \emph{et al.} \cite{goodfellow2014explaining}, we expect to see the adversarialness coming from the linearity of the network \cite{goodfellow2014explaining}, but the decision function given by the softmax will make the output nonlinear.

% UNCOMMENT THIS IN THE FINAL VERSION (ANONYMIZATION)
%We used the Lasagne \cite{lasagne} framework based on Theano \cite{theano} for our experiments, and our code can be found at \hl{add github/bitbucket link.} 

\begin{enumerate}
\item VAEs: encoder and decoder 2 fully connected with 512 neurons each
\item C-VAEs: 
\begin{itemize}
\item MNIST -- ENCODER conv(n filter=32, filter size=4, stride=2), conv(n filter=64, filter size=4, stride=2), conv(n filter=128, filter size=4, stride=2), dense(512) and DECODER dense(512) deconv(n filter=128, filter size=3, stride=2), deconv(n filter=64, filter size=3, stride=2), deconv(n filter=32, filter size=2, stride=2), deconv(n filter=16, filter size=2, stride=2); 
\item SVHN -- ENCODER conv(n filters=32, filter size=4, stride=2), conv(n filters=64, filter size=4, stride=2), conv(n filters=128, filter size=4, stride=2), dense(512) and DECODER dense(512), deconv(n filters=128, filter size=5, stride=2), deconv(n filters=64, filter size=5, stride=2), deconv(n filters=32, filter size=5, stride=2)
\item CelebA -- ENCODER conv(n filters=32, filter size=4, stride=2), conv(n filters=64, filter size=4, stride=2),  conv(n filters=128, filter size=4, stride=2), conv(n filters=256, filter size=4, stride=2), dense(512); DECODER dense(512) deconv(n filters=256, filter size=5, stride=2), deconv(n filters=128, filter size=5, stride=2), deconv(n filters=64, filter size=5, stride=2), deconv(n filters=32, filter size=5, stride=2)
\end{itemize}
\item DRAW:
\begin{itemize}
\item MNIST and SVHN: encoder and decoder lstm(256); MNIST attention read and write 8; SVHN attention read and write 16
\item CelebA: z size 2048, T=1=> enc and dec lstm(2500); others => enc and dec lstm(400); attention read and write 24.
\end{itemize}
\end{enumerate}
For each dataset, six models were trained with two different number of latent variables.  [<=]


\begin{table}
  \caption{Detailed description of the models used}
  \label{tab:models}
  \centering
  \begin{tabular}{l m{4.3cm} m{4.3cm} m{4.3cm}}
    \toprule
              & \multicolumn{3}{c}{Dataset} \\
    \cmidrule(r){2-4}
    Model     & MNIST     & SVHN & CelebA \\
    \midrule
    VAE       & \multicolumn{3}{c}{Encoder and Decoder: fully(512)~$\rightarrow$ fully(512)} \\
    CVAE      &
                % MNIST
                Enc:~conv(32,4)~$\rightarrow$ conv(64,4)~$\rightarrow$ conv(128,4)~$\rightarrow$ fully(512);
                Dec:~fully(512)~$\rightarrow$ dconv(128,3)~$\rightarrow$ dconv(64,3)~$\rightarrow$ dconv(32,2)~$\rightarrow$ dconv(16,2) &
                % SVHN
                Enc:~same as MNIST;
                Dec:~fully(512)~$\rightarrow$ dconv(128,5)~$\rightarrow$ dconv(64,5)~$\rightarrow$ dconv(32,5) &
                % SVHN
                Enc:~conv(32,4)~$\rightarrow$ conv(64,4)~$\rightarrow$ conv(128,4)~$\rightarrow$ conv(256,4)~$\rightarrow$ fully(512);
                Dec:~fully(512)~$\rightarrow$ dconv(256,5)~$\rightarrow$ dconv(128,5)~$\rightarrow$ dconv(64,5)~$\rightarrow$ dconv(32,5) \\
    DRAW      &
                % MNIST
                Encoder and Decoder: LSTM~= 256, attention window~8$\times$8 &
                % SVHN
                Encoder and Decoder: LSTM~= 256, attention window~16$\times$16 &
                % SVHN
                Encoder and Decoder: LSTM~= 2500 (1~timestep) or 400 (16 timesteps), attention window~24$\times$24, latent variables~=2048 \\
    \bottomrule
  \end{tabular}
\end{table}


\begin{table}
  \begin{tabularx}{\textwidth}{|p{0.1\textwidth}|p{0.14\textwidth}|p{0.14\textwidth}|p{0.14\textwidth}|p{0.14\textwidth}|p{0.14\textwidth}|p{0.14\textwidth}|p{0.14\textwidth}|}
    \cline{1-7}
    \multirow{2}{*}{Dataset} &
      \multicolumn{2}{c|}{VAE} &
      \multicolumn{2}{c|}{CVAE} &
      \multicolumn{2}{c|}{DRAW} \\
    & Encoder & Decoder & Encoder & Decoder & Encoder & Decoder \\
    \cline{1-7}
    MNIST & Two FCL with 512 units &  Two FCL with 512 units & 3 CL with filter size 4 and number of filters 32, 64 and 128, followed by a FCL with 512 units & FCL with 512 units followed by 4 DCL with number of filter 128, 64, 32 and 16. The first two with filter size 3 and last two with 2 & LSTM with 256 units and attention window 8x8 & LSTM with 256 units and attention window 8x8 \\
    \cline{1-7}
    SVHN & Two FCL with 512 units & Two FCL with 512 units & 3 CL with filter size 4 and number of filters 32, 64 and 128, followed by a FCL with 512 units &  FCL with 512 units followed by 3 DCL with filter size 5 and number of filters 128, 64 and 32 & LSTM with 256 units and attention window 16x16 & LSTM with 256 units and attention window 16x16 \\
    \cline{1-7}
    CelebA & Two FCL with 512 units & Two FCL with 512 units & 4 CL with filter size 4 and number of filters 32, 64, 128 and 256, followed by a FCL with 512 units & FCL with 512 units followed by 4 DCL with filter size 5 and number of filters 256, 128, 64 and 32 & For the models with 1 timestep and 2048 latent variables, LSTM with 2500 units; for the others LSTM with 400 units. All the attention windows had dimensions of 24x24. & For the models with 1 timestep and 2048 latent variables, LSTM with 2500 units; for the others LSTM with 400 units. All the attention windows had dimensions of 24x24 \\
    \cline{1-7}
  \end{tabularx}
  \caption{[TODO]FCL: Fully-connected layer; CL: Convolutional Layer; DCL: Deconvolutional Layer. All strides were equal to 2.}
\end{table}


